Exploring the different phase diagrams of Strong Interactions

In-medium field-theory is applied to different effective models and QCD to describe mass and isospin effects, finite volume corrections and magnetic fields in the phase diagram of Strong Interactions, keeping close contact with experiments and lattice results. Findings range from a technical nonperturbative solution of the hot and dense regime of a general massive Yukawa Theory and the computation of the cold and dense chiral surface tension -- a key quantity for supernovae explosions and compact star structure -- to the proposal of a novel signature for the QCD critical endpoint in heavy-ion collisions based on finite-size scaling. The behavior of the deconfining critical temperature as a function of the pion mass and the isospin chemical potential is also addressed in an effective model and the description obtained is in agreement with lattice simulations, in contrast to what is found in (Polyakov-extended) chiral models. We also discuss the thermodynamics of QCD in the presence of a (Abelian) magnetic field to two-loop order and a Functional-Renormalization-Group analysis of relativistic Bose-Einstein condensation of pions in isospin-dense media.

==> apresentacao.tex <==
\chapter{apresentacao}

\be 
&&Z=\int\mathcal{D}\sigma\,\mathcal{D}\vec{\pi}\;\left\{\exp\left[-\int_x\left(\frac{1}{2}\partial_\mu\phi\partial_\mu\phi+V\left(\phi\right)\right)\right]\times\white\right\}\nonumber\\
&&\sp\;\;\;\;\;\;\;\;\;\;\white\left\{\black\times det\left[\left(p_\mu\gamma_\mu-\mu\gamma^0-g(\sigma+i\gamma_5\vec{\tau}\cdot\vec{\pi})\right)/T\right]\right\}\,\black,
\ee

\be
\frac{d^2\phi}{dr^2}+\frac{3}{r}\frac{d\phi}{dr}=V_{ef}'(\phi)\,\,\,.
\ee

\be
r=(\tau^2+|\vec{x}|^2)^{1/2}\,\,\,,
\ee

\be
\lim_{r\rightarrow\infty}\phi(r)=0\,\,\,.
\ee

\begin{equation}
\phi_c(r;\xi,r_c)=\phi_f+\frac{1}{\xi\sqrt{2\alpha}}\left[1-\tanh\left(\frac{r-r_c}{\xi}\right)\right]\,\,\,,
\end{equation}

\begin{equation}
V_{in}\approx\sum_{n=0}^4a_n(T)\,\phi^n\,\,\,.
\end{equation} 

==> titulo.tex <==
\begin{titlepage}

\vspace*{13.5cm}

\centerline{{\huge EXPLORING THE}} 

\vspace*{0.7cm}

\centerline{{\huge DIFFERENT PHASE DIAGRAMS}} 

\vspace*{0.7cm}

\centerline{{\huge OF STRONG INTERACTIONS}}


\vspace*{2.3cm}

{\bf LET\'ICIA FARIA DOMINGUES PALHARES}
\end{titlepage}

